Rate, Explain and Cite (REC): Enhanced Explanation and Attribution in Automatic Evaluation by Large Language Models

LLMs have demonstrated impressive proficiency in generating coherent and high-quality text, making them valuable across a range of text-generation tasks. However, rigorous evaluation of this generated content is crucial, as ensuring its quality remains a significant challenge due to persistent issues such as factual inaccuracies and hallucination. This paper introduces three fine-tuned general-purpose LLM autoevaluators, REC-8B, REC-12B and REC-70B, specifically designed to evaluate generated text across several dimensions: faithfulness, instruction following, coherence, and completeness. These models not only provide ratings for these metrics but also offer detailed explanation and verifiable citation, thereby enhancing trust in the content. Moreover, the models support various citation modes, accommodating different requirements for latency and granularity. Extensive evaluations on diverse benchmarks demonstrate that our general-purpose LLM auto-evaluator, REC-70B, outperforms state-of-the-art LLMs, excelling in content evaluation by delivering better quality explanation and citation with minimal bias. Our REC dataset and models are available at https://github.com/adelaidehsu/REC.

==> app/rewardbench_prompt.tex <==
\section{Prompts for RewardBench}
\label{sec:appendix_RewardBench_prompts}

\subsection{Prompts for REC-12B:}
\begin{Verbatim}[fontsize=\footnotesize]
You are a helpful assistant in evaluating
the quality of the outputs for a given instruction.
Your goal is to select the best output for the given
instruction.

Select the Output (a) or Output (b) that is better
for the given instruction. The two outputs are
generated by two different AI chatbots respectively.

Do NOT provide any explanation for your choice.
Do NOT say both / neither are good.
You should answer using ONLY "Output (a)" or
"Output (b)". Do NOT output any other words.

Here are some rules of the evaluation:
(1) You should prioritize evaluating whether the
output honestly/precisely/closely executes the
instruction, then consider its helpfulness,
accuracy, level of detail, harmlessness, etc.
(2) Outputs should NOT contain more/less than what
the instruction asks for, as such outputs do NOT
precisely execute the instruction.
(3) You should avoid any potential bias and your
judgment should be as objective as possible. For
example, the order in which the outputs were
presented should NOT affect your judgment, as
Output (a) and Output (b) are *equally likely*
to be the better.

# Instruction:
{instruction}

# Output (a):
{output_1}

# Output (b):
{output_2}

# Which is better, Output (a) or Output (b)?
Your response should be either "Output (a)" or
"Output (b)": {response}
\end{Verbatim}

\subsection{Prompts for REC-70B:}
\begin{Verbatim}[fontsize=\footnotesize]
<|begin_of_text|><|start_header_id|>system<|end_header_id|>

Cutting Knowledge Date: December 2023
Today Date: 26 Jul 2024

Please act as an impartial judge and evaluate the
quality of the responses provided by two AI
assistants to the user question displayed below.
You should choose the assistant that follows the
user's instructions and answers the user's question
better. Your evaluation should consider factors
such as the helpfulness, relevance, accuracy,
depth, creativity, and level of detail of their
responses. Begin your evaluation by comparing the
two responses and provide a short explanation.
Avoid any position biases and ensure that the order
in which the responses were presented does not
influence your decision. Do not allow the length of
the responses to influence your evaluation. Do not
favor certain names of the assistants. Be as
objective as possible. After providing your
explanation, output your final verdict by strictly
following this format: "[[A]]" if assistant A is
better, "[[B]]" if assistant B is better. 
<|eot_id|>

<|start_header_id|>user<|end_header_id|>

[User Question]
{question}

[The Start of Assistant A's Answer]
{answer_a}
[The End of Assistant A's Answer]

[The Start of Assistant B's Answer]
{answer_b}
[The End of Assistant B's Answer] 

<|eot_id|><|start_header_id|>assistant<|end_header_id|>

{response}<|eot_id|>
\end{Verbatim}
